Designing Optimal Personalized Incentive for Traffic Routing using BIG Hype algorithm

We study the problem of optimally routing plug-in electric and conventional fuel vehicles on a city level. In our model, commuters selfishly aim to minimize a local cost that combines travel time, from a fixed origin to a desired destination, and the monetary cost of using city facilities, parking or service stations. The traffic authority can influence the commuters' preferred routing choice by means of personalized discounts on parking tickets and on the energy price at service stations. We formalize the problem of designing these monetary incentives optimally as a large-scale bilevel game, where constraints arise at both levels due to the finite capacities of city facilities and incentives budget. Then, we develop an efficient decentralized solution scheme with convergence guarantees based on BIG Hype, a recently-proposed hypergradient-based algorithm for hierarchical games. Finally, we validate our model via numerical simulations over the Anaheim's network, and show that the proposed approach produces sensible results in terms of traffic decongestion and it is able to solve in minutes problems with more than 48000 variables and 110000 constraints.

==> commands.tex <==
%% Math Symbols
\newcommand{\setR}{\mathbb{R}}
\newcommand{\setN}{\mathbb{N}}
\newcommand{\setRp}{\setR_{\geq 0}}
\newcommand{\setRn}{\setR_{\leq 0}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\tup}[1]{\textup{#1}}
\newcommand{\ball}{\mathcal{B}}
\newcommand{\ones}{\boldsymbol{1}}
\newcommand{\bolds}[1]{\boldsymbol{#1}}
\newcommand{\abs}[1]{\left| #1 \right|}
%\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\proj}[1]{\mathbb{P}_{#1}}
\newcommand{\indic}[1]{\mathcal{I}_{#1}}
\newcommand{\inner}[2]{\left\langle #1 , \,  #2 \right\rangle}
\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\tderiv}[2]{\frac{d #1}{d #2}}
\newcommand{\jac}{\boldsymbol{\mathrm{J}}}
\newcommand{\clarke}{\jac^c}
\newcommand{\conserv}{\boldsymbol{\mathcal{J}}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\blkdiag}{blkdiag}
\DeclareMathOperator{\col}{col}
\DeclareMathOperator{\spanop}{span}
\DeclareMathOperator{\inter}{int}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\bnd}{bnd}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\ncone}{N}
\DeclareMathOperator{\spec}{\textsc{Spec}}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\Jac}{Jac}
\DeclareMathOperator{\Jacc}{Jac^{\,c}}
\DeclareMathOperator{\sol}{SOL}
\DeclareMathOperator{\vi}{VI}
\DeclareMathOperator{\fix}{fix}

% Problem Formulation
\newcommand{\agents}{\mathcal{N}}
\newcommand{\cy}{\bolds{y}}
\newcommand{\cys}{ \cy^{\star} }
\newcommand{\csigma}{\bolds{\sigma}}
\newcommand{\cw}{\conc{w}}
\newcommand{\com}{\conc{\omega}}
\newcommand{\polyset}{\ml{N}_p}
\newcommand{\clambda}{\conc{\lambda}}
\newcommand{\cnu}{\conc{\nu}}

% Energy Markets
\newcommand{\phires}{\phi^{\textrm{R}}}
% Incentive rebound
\newcommand{\pireb}{\pi^{\textrm{B}}}
% Incentive  response
\newcommand{\pires}{\pi^{\textrm{R}}}
\newcommand{\piresnet}{\pi^{\textrm{net,R}}}
% Charing power
\newcommand{\picha}{p^{\textrm{C}}}
\newcommand{\pidisch}{p^{\textrm{DC}}}

% Environment Names
\newtheorem{definition}{Definition}
\newcommand{\definitionautorefname}{Definition}
\newtheorem{lemma}{Lemma}
\newcommand{\lemmaautorefname}{Lemma}
\newtheorem{proposition}{Proposition}
\newcommand{\propositionautorefname}{Proposition}
\newtheorem{remark}{Remark}
\newcommand{\remarkautorefname}{Remark}
%\renewcommand*{\thestassumption}{\Alph{stassumption}}

\usepackage[acronym]{glossaries}
\newacronym{SoC}{SoC}{State of Charge}
\newacronym{PEV}{PEV}{Plug-in Electric Vehicle}
\newacronym{EV}{EV}{Electric Vehicle}
\newacronym{FV}{FV}{fuel vehicle}
\newacronym{TA}{TA}{Traffic Authority}
\newacronym{VRP}{VRP}{Vehicle Routing Problem} 
\newacronym{TTT}{TTT}{Total Travel Time} 
\newacronym{NE}{NE}{Nash equilibrium}
\newacronym{PG}{PG}{Pseudo-Gradient}
\newacronym{BIG Hype}{BIG Hype}{Best Intervention in Games using Hypergradients}
\newacronym{VI}{VI}{Variational Inequality}

% Define the algorithm environment
% Create Algorithm Environment
\newcounter{algorithm}
\newenvironment{algorithm}[1][]
{	\refstepcounter{algorithm}
	\begin{minipage}{\linewidth}
		\medskip
		\hrule
		\smallskip
		\textsc{Algorithm \thealgorithm}. #1
		\smallskip
		\hrule 
		\smallskip
	\end{minipage}
}
{
	\smallskip
	\hrule width\linewidth\relax
	\smallskip
}
\newcommand{\algorithmautorefname}{Alg.}
\newcommand{\CC}[1]{{\color{magenta}#1}}






